Obsidian: Cooperative State-Space Exploration for Performant Inference on Secure ML Accelerators

Trusted execution environments (TEEs) for machine learning accelerators are indispensable in secure and efficient ML inference. Optimizing workloads through state-space exploration for the accelerator architectures improves performance and energy consumption. However, such explorations are expensive and slow due to the large search space. Current research has to use fast analytical models that forego critical hardware details and cross-layer opportunities unique to the hardware security primitives. While cycle-accurate models can theoretically reach better designs, their high runtime cost restricts them to a smaller state space. We present Obsidian, an optimization framework for finding the optimal mapping from ML kernels to a secure ML accelerator. Obsidian addresses the above challenge by exploring the state space using analytical and cycle-accurate models cooperatively. The two main exploration components include: (1) A secure accelerator analytical model, that includes the effect of secure hardware while traversing the large mapping state space and produce the best m model mappings; (2) A compiler profiling step on a cycle-accurate model, that captures runtime bottlenecks to further improve execution runtime, energy and resource utilization and find the optimal model mapping. We compare our results to a baseline secure accelerator, comprising of the state-of-the-art security schemes obtained from guardnn [ 33 ] and sesame [11]. The analytical model reduces the inference latency by 20.5% for a cloud and 8.4% for an edge deployment with an energy improvement of 24% and 19% respectively. The cycle-accurate model, further reduces the latency by 9.1% for a cloud and 12.2% for an edge with an energy improvement of 13.8% and 13.1%.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png

.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*


.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> Security_analysis.tex <==
\section{Security Analysis and Evaluation}

\sys{} framework relies on several compiler optimizations and secure hardware components.
The key components ensuring security across the \sys{} stack are listed in ~\cref{fig:sec_anal}.
In this section, we argue how the security guarantees mentioned in ~\cref{subsec:sec_prop} is preserved during compilation, tenant bootstrapping and execution. 

\begin{figure}[hbtp]
    \centering
    \includegraphics[width=0.8\linewidth]{Figures/security_analysis.pdf}
    \vspace{-1em}
    \caption{\textbf{Security guarantees across the \sys{} stack}}
    \label{fig:sec_anal}
\end{figure}
% \vspace{-1em}

\subsection{Data protection during model compilation}
The model owner defines the ML model topology and weights with model declaration APIs. 
The APIs and the compiler code are downloaded from the official website and the binary is verified before installation. 
The \sys{} compiler is part of our trusted computing base (TCB). 
% Formal verification of the \sys{} compiler will be done in the future. 

Application profiling is carried out in a platform with the same security policies as the execution.
The application is run multiple times during profiling.
Since \sys{} hardware ensures complete execution isolation for a single ML inference, we argue that running the application multiple times do not reveal any additional information.

% \vspace{-0.5em}
\subsection{Data protection during tenant bootstrapping}
A trusted SK firmware is loaded through secure boot and it prepares the device attestation report signed with a private key stored in a secure storage. 
The tenant verifies the device through remote attestation and sends the tenant configuration and confidential model data over a secure channel.
The SK firmware has exclusive access to write the tenant configuration in hardware registers.
%It additionally loads the encryption and integrity keys to the respective hardware units and loads the model binary in memory.
We assume the SK firmware is a part of \sys{} TCB and restrict any other software from accessing accelerator configuration registers and key storage.
The same interface is used to load the inference input data.

% \vspace{-0.5em}
\subsection{Unique key for each tenant}
The encryption and the integrity keys are generated from a pseudo-random number generator during the compiler stage. 
\sys{} compiler encrypts the secret model data using the encryption key and the MAC is generated with the integrity key. 
These keys are unique for each tenant and are loaded by SK in a secure storage, mapped with the tenant session ID. 
Having unique keys for each tenant prevents an attacker from violating the victim data confidentiality (S2) and integrity (S3). 

% \vspace{-1em}
\subsection{Secure execution guarantees}
The hardware security widgets ensuring isolated execution is shown in ~\cref{fig:sec_anal}.
Data value confidentiality (\texttt{S1}) and integrity (\texttt{S2}) guarantees are ensured in memory by storing encrypted data along with MAC. 
The page table storing the base address and size of tenant memory allocation is inaccessible to other tenants, safeguarding data structure confidentiality (\texttt{S3}). 
%Data tampering in memory bus will be detecting by integrity verification. 
The memory shaper preserves the \texttt{S3} guarantee by obfuscating demand traffic variations in both read and write bus.

An attacker has no access to on-chip resources during temporal sharing, while the micro-architectural buffers and the compute unit is partitioned during spatial sharing.
Instruction, dependency and compute buffers are statically partitioned during spatial sharing. 
Same is done for metadata caches, the request and the staging buffers. 
The scratchpad regions are access-controlled for each tenant, protecting \texttt{S1,S2} and \texttt{S3} guarantees. 
Finally, the secret data in the scratchpad is zeroized to remove any data before context switching. 

 \begin{table}[t]
     \resizebox{\linewidth}{!}{%
    \begin{tabular}{lccccccc}
        \toprule
        \textbf{Benchmark} & \textbf{Alexnet} & \textbf{Resnet50} & \textbf{FasterRCNN} & \textbf{DLRM} & \textbf{AlphaGoZero} & \textbf{Translate} & \textbf{Transformer} \\
        \midrule
         \textbf{Layer} &  \large\multirow{2}{*}{$100\%$} &  \large\multirow{2}{*}{$90.3\%$} &  \large\multirow{2}{*}{$88.5\%$} &  \large\multirow{2}{*}{$70.9\%$} &  \large\multirow{2}{*}{$91.0\%$} &  \large\multirow{2}{*}{$62.5\%$} &  \large\multirow{2}{*}{$46.2\%$}  \\
         \textbf{Classification} & & & & & & & \\
        \bottomrule
    \end{tabular}
}
    \caption{\textbf{Percentage of model layer sizes classified by a CNN model by observing the memory bandwidth.}}
    \label{tbl:shaper}
    % \input{Tables/tee_comparison.tex}
   % \vspace{-1em}
\end{table}

\begin{comment}
    

\footnotesize
\begin{tabular} {lrrrr}
\toprule
% {\bf Coverage} 
\multirow{2}{*}{\textbf{Layer Classification}} & \multicolumn{2}{c}{\textbf{Arm platform}} &\multicolumn{2}{c}{\textbf{x86 platform}} \\
\cmidrule(r){2-3} \cmidrule(l){4-5}
& \textbf{Auditd-IM} & \textbf{\sys} & \textbf{Auditd-IM} & \textbf{\sys} \\
\midrule
{NGINX} &  5270 & 5624 &23471 & 23724  \\
% \hline
\bottomrule
%\textbf{get_pid} & 64095 & 345.3 & 156844 & 60.1   \\
%\hline
%\textbf{Geomean} & \textbf{9372} & \textbf{286.0} & \textbf{11120}, \textbf{46.9} \\
\end{tabular}
\end{comment}
% \vspace{-0.5em}
\subsection{Effectiveness of the memory traffic shaper}
The attacker should not be able to violate \texttt{S3} by observing the shaped output.
To understand the security implication of the traffic shaper, we build a CNN classifier to predict the ML layers with the memory bandwidth trace. 
We assume a powerful attacker, has complete access to the exact memory bandwidth.
Similar to prior work~\cite{band_util}, we identify the layer boundary followed by the layer size.
The first step is identifying the layer tile boundary.
Each tile computes a matrix-vector or matrix-matrix computation with the output feature map being written back to memory. 
This write transaction is used to detect a layer tile boundary. 
The read bandwidth trace is split into tile boundary intervals.
The layer matrix size is extracted from read bandwidth variations for each tile.

We ran each benchmark 50 times and split each trace at the tile boundary, to craete the training dataset.
Next, we use discrete wavelet transform (DWT) on the read bandwidth signature for each tile. 
Different layer bandwidth traces vary in execution length, but applying DWT produces a fixed-sized feature.
We use a 3-layer convolutional neural network (CNN) to classify the DWT trace. 
This model is trained with categorical crossentropy in keras, with $70\%$ training data and $30\%$ validation data. 
~\cref{tbl:shaper} shows the percentage of layer sizes identified by the CNN model for unshaped traffic. 
For simpler models with non-uniform adjacent layers like \textit{Alexnet}, our classifier achieves perfect layer structure classification. 
The Classifier performs poorly for models with similar adjacent layers like \textit{Translate} and \textit{Transformer}.
But, even in the worst case, the attacker is able to decipher $46.2\%$ of layers structures through bandwidth observation. 

The classifier fails to identify layer boundaries due to
constant shaping of the write bus. 
The attacker observes a fixed-size write transaction at regular intervals. 
The round-robin bank arbitration prevents the attacker from distinguishing between a real and a fake transaction. 
Moreover, the read bus bandwidth is constant and is independent of the tile size, thus preventing our classifier from violating the S3 security guarantee.
% \vspace{-0.5em}

\subsection{Replay attacks on read-only model data}
\sys{} eliminates integrity counters for read-only ML models as a part of data integrity optimization. 
The MAC scheme still protects against replay attacks. 
The \sys{} compiler assigns a fixed address to each model data. 
During deployment, the SK allocates a memory region and stores the ML model in the same sequence. 
The relative address of each model weight can be computed by subtracting the deployment base address and is used for MAC verification.
This scheme provides replay protection, as long as, the relative address of each model weight remains unchanged.
Given that the values of model weights do not changed during execution, any memory tampering will trigger data integrity failure.



==> code.tex <==
\definecolor{codegreen}{rgb}{0,0.6,0}
\definecolor{codegray}{rgb}{0.5,0.5,0.5}
\definecolor{codepurple}{rgb}{0.58,0,0.82}
\definecolor{backcolour}{rgb}{0.95,0.95,0.95}

\lstdefinestyle{mystyle}{
    backgroundcolor=\color{backcolour},   
    commentstyle=\color{codegreen},
    keywordstyle=\color{magenta},
    numberstyle=\tiny\color{codegray},
    stringstyle=\color{codepurple},
    basicstyle=\ttfamily\footnotesize,
    breakatwhitespace=false,         
    breaklines=true,                 
    captionpos=b,                    
    keepspaces=true,                 
    numbers=left,                    
    numbersep=5pt,                  
    showspaces=false,                
    showstringspaces=false,
    showtabs=false,                  
    tabsize=2
}

\lstset{style=mystyle}
\begin{lstlisting}[language=Python, caption=Sample code for addition of two secret matrices]
import numpy as np
from tvm import te
n = 1024
#Define the deployment configuration
sec_pragma(exec_mode ="spatial", inte_gran=1024)
res_pragma(mem_bw=0.25, spad=0.25, comp=0.25)
#Secret model weights and topology
mod = te.placeholder((n,n), name="mod",
    encr=1, inte=1, shap=1)  
#Define secret input region
x_range = np.array(start=50, stop=60)
y_range = np.array(start=20, stop=30)
#Partial input secret
inp = te.placeholder((n,n), name="inp",encr=1, inte=1, shap=1, x_conf=x_range, y_conf=y_range) 
#Performing vector addition
out = te.compute(mod.shape, 
lambda i: mod[i] + inp[i], name="out")
\end{lstlisting}


==> compiler.tex <==
\section{\sys{} design}

\begin{comment}
    

\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/analytical_steps.drawio.pdf}
    \caption{\textbf{The analytical model for a secure ML inference accelerator}}
    \vspace{-1em}
    \label{fig:analytical_model}
    \end{figure}

The main components of \sys{} design 

\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/tenant_zero_flow.pdf}
    \caption{\textbf{The \sys{} software includes \textit{(1) Model declaration} using specialized APIs; 
    \textit{(2) Compiler transformations} to optimize secret propagation;
    \textit{(3) Application profiling} of security defence mechanisms;
    And \textit{(4) code generation} to program the optimized configuration in accelerator hardware and execute the model binary.
    }}
    \vspace{-1em}
    \label{fig:tenant_zero_flow}
    \end{figure*}
    \end{comment}
The first optimization is to reduce the resident secret data in scratchpad during context switch.
\sys{} performs data liveness analysis to find the last compute access for each data.
Once, the data is expired, the specific scratchpad location is zeroized and if dirty, written back to memory. 
This zeroization operation is interleaved with regular computation, leveraging the decoupled access-execute nature of the architecture.
We call this technique as \textit{proactive zeroization}.

The second optimization replaces fake transaction intervals of a traffic shaper with cross-tile or cross-layer data prefetches.
The proactive zeroization increases the opportunity for new data prefetches by clearing dead variables from the scratchpad.

\sys{} further decides the granularity of MAC verification of each model layer as a third optimization. 
We observe the optimal MAC granularity depends on the application layer tile size, access sequence, stride and other parameters.

\subsection{Dataflow mapping}
\label{subsec:dataflow}
The scheduling of compute operations is critical for obtaining a reasonable inference performance. 
Prior work~\cite{maestro,timeloop} used analytical model of ML inference computation to find the optimal scheduling. 
Given the static nature of ML inference, the analytical models have good correlation with real executions.
The existing solutions are designed for non-secure ML inference, with hardware specifications including the number of processing units (PE), scratchpad size, NOC and memory bandwidth. 
However, these models do not capture the additional interactions by the secure hardware primitives.

In this work, we extend the maestro~\cite{maestro} analytical model to include a traffic shaper, an authenticated encryption block and a zeroize module as shown in green boxes in Figure~\cref{fig:analytical_model}.
\sys{} analytical model takes hardware and model specification as input.
The model specification specifies the layer topology and size, defined in the same format as in Maestro. 
The hardware specification is augmented to include the properties of the secure primitives.
The traffic shaper is modeled as a queue that sends a transaction at a fixed interval.
There are separate queues for read and write traffic and the fixed interval is specified by the tenant allocated memory bandwidth in the hardware specification.
The authenticated encryption unit is modeled as a constant throughput cryptographic engine, similar to secureloop~\cite{secureloop}.
However, secureloop studies different cryptographic engines, but we consider the pipelined \textit{aes-gcm} implementation~\cite{aesPipeline} in our evaluation, which has the least overhead. 
Finally, \sys{} has a zeroize module that models the cost of tenant context switch. 

The analytical model outputs the top-k optimal dataflow mapping for each layer.
Additionally, the traffic shaping module outputs the ratio of fake transactions for each dataflow,
the authenticated encryption module finds the optimum integrity granularity, 
and the zeroize module reports the context switch latency. 
These reports are used in the next optimization steps.

\begin{comment}
It counts the number of scratchpad lines filled with secret data at each layer boundary and reports the time needed to zeroize these locations.
The analytical model outputs the optimal dataflow mapping, given a hardware and a model specification. The cost analysis algorithm finds the 


Maestro already models a DRAM with a memory bandwidth, the scratchpads and the systolic array model with sizes specified in the hardware specification. 

Secureloop~\cite{secureloop} captures the effect of a crypto engine performing authenticated encryption. 
For the 
Moreover, we look into temporal and spatial multi-tenant accelerators, where a multiple tiles can execute into parallel spatial partitions to leverage parallelism. 

Figure~\cref{fig:analytical_model} shows the various components of a secure ML accelerator. 
Maestro~\cite{maestro} builds an analytical model 

\end{comment}

\subsection{Dataflow to layer binary generation}
\subsection{Proactive scratchpad zeroization}
Ensuring a stateless accelerator during context switch prevent side-channel leaks between distrustful tenants.
The analytical model described in ~\cref{subsec:dataflow} reports the zeroize latency for each layer. 
This zeroize latency includes writing zeros in secret scratchpad locations
and memory writeback of dirty data from the output scratchpad.

We aim to reduce the context switch latency by interleaving zeroization with the layer computation.
This requires tracking the data dependencies in the scratchpads. 
Secrets resident in input and weight scratchpads must be consumed by the compute unit before zeroization. 
Similarly, the secrets, generated by the compute unit should be queued for storing before output zeroization. 
\sys{} compiler computes the reuse distance of each secret data.



The execution schedule should ensure two properties: \textbf{(1)} Every data should be consumed by the compute unit before it is zeroized and; \textbf{(2)} Data exhibiting temporal locality should not be zeroized. 
The first property is important for functional correctness of the inference execution while the second one improves execution performance. 
We solve both this problems by incorporating a variable reuse analysis pass in the compiler. 

The reuse analysis takes the compute schedule as input and finds the reuse distance of each variable. 











In this section, we discuss the components of \sys{} software stack from model definition APIs, compiler transformation, and profiling, to model binary and secure hardware configuration generation.
\vspace{-0.5em}
\subsection{\sys{} software stack primitives}
~\cref{fig:soft_arch} shows the different components of the \sys{} compiler. 
A developer uses the model declaration API to define the ML model and the deployment specification as discussed in ~\cref{subsec:apis}.
The compiler transforms the ML model into a dataflow graph. 
Compiler optimizations like data liveness analysis and fake traffic reduction, harness application characteristics to reduce inference latency, while application profiling optimizes the tile size for each layer and the MAC computation granularity (\cref{subsec:compiler_passes}).
%Application profiling optimizes , etc.  (~\cref{subsec:profiling}).
The code generation includes accelerator configuration, which is programmed to hardware registers during tenant bootstrapping and the model binary.

\begin{comment}
\sys{} software takes security and resource declaration from model developer as input and generates optimized code for secure ML inference. 
In this section, we introduce the model declaration APIs (~\cref{subsec:apis}) to declare secret 
variable attributes and platform resource declaration. 
Next, we detail the compiler transformations and the performance optimization passes in ~\cref{subsec:compiler_passes};
Multiple execution parameters are profiled to tune the application for low latency inference. (~\cref{subsec:profiling}).
Finally, we discuss how the optimized binary communicates the security attributes of each variable to the hardware with the help of ISA extensions.
\end{comment}
%\input{code}
\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/soft_arch.pdf}
    \caption{\textbf{The \sys{} software includes \textit{(1) Model declaration} using specialized APIs; 
    \textit{(2) Compiler transformations} to optimize secret propagation;
    \textit{(3) Application profiling} of security defence mechanisms;
    And \textit{(4) code generation} to program the optimized configuration in accelerator hardware and execute the model binary.
    }}
    \vspace{-1em}
    \label{fig:soft_arch}
    \end{figure}
%\vspace{-1em}
\subsection{Model declaration APIs}
\label{subsec:apis}
\sys{} uses TVM~\cite{tvm} APIs to define the model topology and the deployment parameters. 
Model and input variables are defined using the TVM tensor expression (te) API~\cite{tvm_te}. 
Each tensor is initialized by the \textit{te.placeholder()} function. 
By default, this function takes a variable name, size, and datatype as arguments.
\sys{} adds a new \texttt{ro} argument to indicate read-only tensors.
This reduces metadata memory traffic by eliminating integrity counters used for replay protection.
Keeping the application frontend coherent with TVM enables the user to define models using Tensorflow~\cite{tensorflow}, Keras~\cite{keras}, Pytorch~\cite{pytorch}, and use trained models from Model Zoos~\cite{model_zoo}.

Deployment definition provides the hardware and tenancy specification for an application.
The inference execution allocates accelerator resources and isolate the tenant based on this specification.
%It is additionally used to reserve upfront accelerator resources and isolate the execution. 
The resource and tenancy requirement is defined with specialized pragmas.
These pragmas define multi-tenancy mode (spatial or temporal sharing) and the compute resource allocation including scratchpad, buffers, compute units and memory bandwidth quotas.
The accelerator hardware writes these into tenant configuration registers during bootstrapping.
\vspace{-1em}
\subsection{Compiler transformations and profiling}
\label{subsec:compiler_passes}
The TVM parser parses the new pragmas and tensor attributes. 
The ML model is transformed into a dataflow graph.
Graph transformation and functional optimizations are performed with existing TVM compiler passes. 
%Moreover, hardware register writes are generated for tenant allocation.
Optimization of security primitives, including data liveness analysis and reduction of fake transactions in the memory traffic shaper is added to the compiler to reduce latency overhead. 

 
\subsubsection{Data liveness analysis}
\label{subsec:liveness}
\sys{} compiler performs data liveness analysis to identify and remove dead variables immediately after the last access. 
The scratchpad locations, holding dead variables are over-written with zeros with a new \texttt{zeroize} instruction.
These instructions are added to the model binary based on this analysis.
The compiler creates an execution sequence based on the dataflow graph.
This compiler pass re-orders the parallel nodes of the dataflow graph to maximize data locality. 
The variable reuse distance is analyzed, and dead variables are cleared using the \texttt{zeroize} instruction.
%The secret data inputs to a graph node are zeroized, right after the compute instruction.
%This compiler pass, further uses these free scratchpad regions to perform early-load of subsequent model layers.
Subsequent load instructions, which do not have data dependencies, are promoted to fill into these free scratchpad regions.
%Clearing dead variables proactively frees up the scratchpad, which is used to promote data loads for later tiles.
This optimization leads to better memory bandwidth utilization, leading to fewer memory stalls, during high demand traffic.
Moreover, data liveness analysis reduces the tenant context switch overhead by reducing the volume of left-over secrets and is evaluated in ~\cref{subsec:eval_zeroize}.

\subsubsection{Fake memory traffic reduction}
\sys{} hardware has a constant traffic shaper (discussed in ~\cref{subsec:shaper}), which moderates the memory demand transactions to create a constant traffic in the memory bus. 
The shaper throttles high bandwidth demand requests, while fake transactions are sent over the memory bus, when the memory request queue is empty.
Leveraging liveness analysis, the \sys{} compiler substitutes some of these fake transactions to pre-load the next layer in vacant scratchpad regions.
In the absence of free scratchpad locations, the compiler promotes the integrity metadata load transactions.
\sys{} generates the integrity MAC and counters in the compiler, so that they can be resident in dedicated metadata caches before the real data transaction.
Replacement of fake transactions by reordering real transactions, improves overall inference latency as evaluated in ~\cref{subsec:eval_shaper}.

%\vspace{-0.5em}

\subsubsection{Model layer tiling}
Each layer is profiled with multiple tile sizes that fit in the allocated scratchpad. 
The dataflow graph is split into tile size having the best inference latency. 
Model tiling, not only depends on the scratchpad and compute unit allocation, but also on the
shaper bandwidth allocation and the throughput of the encryption and the integrity unit.

\subsubsection{Application integrity granularity}
\label{subsec:inte_gran}
\sys{} integrity engine is designed to verify MAC at a configurable granularity, ranging from $64B$ to $4kB$. 
The granularity depends on the model layer size and this profiling step is used to find the optimal one.
Having an integrity granularity of $64B$ will increase the number of MAC calculations and the metadata memory traffic.
However, it works great with strided matrices or smaller layers.
If a tensor is smaller than the MAC granularity, the entire data has to be loaded to perform MAC verification, leading to wasted memory traffic. 
However, large continuous data loads work best with a larger granularity due to less MAC computation and memory traffic overhead from metadata transactions.
Each application is profiled to find the optimum integrity granularity for the entire application. 
The compiler adds a configuration register write in the binary to program the MAC granularity. 
The performance improvements from integrity granularity adjustment are demonstrated in~\cref{subsec:eval_integrity}.



%The TVM compiler converts the ML model into a dataflow graph. 
%The edges of the graph represents data variables and the node represents the compute operation. 
%This compiler pass extracts the time 


==> design.tex <==
% \vspace{-0.5em}
\section{\sys{} Hardware Architecture}
%-------------------------------------------------------------------------------
\label{sec:overview}
%\vspace{-1em}

    
This section first provides an overview of the \sys{} design primitives
in~\cref{subsec:primitives},
tenant bootstrapping in~\cref{subsec:secure_kernel}, 
illustrate the execution flow in~\cref{subsec:exec_flow},
and finally describe the additional secure hardware required
in~\cref{subsec:mem_proc_eng,subsec:shaper,subsec:zeroize}.
In summary, \sys{} offer primitives for memory isolation, encryption and integrity protections,
off-chip memory bandwidth protection and on-chip resource isolation.

% \vspace{-0.5em}
\subsection{Hardware defence primitives}
\label{subsec:primitives}
%\vspace{-1em}

\quad \textbf{On-chip resource partitioning:}
Several distrustful tenants can share and execute concurrently in the accelerator to improve utilization in the spatial sharing mode.
Attackers can launch timing, utilization and contention side-channels on the victim.
\sys{} eliminates these channels by statically partitioning on-chip scratchpad, adders and multipliers in compute units and micro-architectural queues (instruction, dependency and memory buffers) for each tenant during bootstrapping.
This results in complete data and timing isolation,
limiting the attacker's observation into victim resources. 

\textbf{Left-over state zeroization:}
Secret data resides as plaintext in on-chip scratchpad and other buffers.
Each secret location is overwrriten with zero before context switch, preventing use-after-free attacks.
However, clearing the entire scratchpad has a significant overhead.
Data liveness analysis interleaves zeroization with computation to reduce the left-over state during context switch.
This is implemented with a hardware module, issuing the \texttt{zeroize} instructions in parallel to the compute and memory execution.

\textbf{Memory protection:}
Memory protection includes encryption, integrity verification and access control of tenant scratchpad regions.
Secret data is stored in an encrypted format outside of the accelerator.
Authenticated encryption protocols (e.g., AES-GCM) protect data confidentiality and integrity, both at-rest and during transit between the off-chip storage and the accelerator.
A secure key storage holds unique encryption and integrity keys for each tenant.
The key storage is only accessible by the secure firmware.
The tenant scratchpad regions are access-controlled for each tenant. 
Each compute operation undergoes scratchpad base and bound address check to prevent buffer overflow attacks and other memory safety violations.


% In certain scenarios like public clouds, data integrity can also be provided as a part of service level agreement (SLA) with no malicious agent having physical access to the datacenters.
%    There is no need to protect integrity cryptographically in those cases.
%The tenant off-chip memory regions as well as scratchpad allocations are access-controlled through a permission table, programmed at tenant provisioning time.

\textbf{Memory bandwidth shaping:}
Memory traffic shaping logic obfuscates bandwidth variations on the memory bus.
% Prior works~\cite{band_util} demonstrated how an attacker can sample bandwidth utilization to find matrix sizes for each ML layer.
\sys{} incorporates a constant memory bandwidth shaping logic to prevent such attacks. 
Each memory requests are split into constant sized bursts and sent to the memory controller at regular intervals. 
Memory requests are padded to be a multiple of the burst size. 
Requests are throttled in the memory controller when the demand exceeds the allocated bandwidth,
while fake transactions are injected otherwise.

%\vspace{-0.5em}
\subsection{Secure Kernel (SK)}
\label{subsec:secure_kernel}
 
%to --- send device attestation report to the tenants over a TLS session; 
%receive model and data values for inference; and finally program the configuration registers based on the execution requirement.
The \sys{} secure kernel is the root-of-trust of the system.
The SK trusted firmware can be implemented in a small micro-controller for
accelerator bootstrapping,
and performs remote attestation with the tenants.
The SK firmware is loaded during secure boot and it initializes the accelerator platform.
A tenant can only communicate with the accelerator through a limited interface provided by the SK.

Steps \circled{1} to \circled{5} in \cref{fig:hw_arch} illustrate tenant bootstrapping.
\circled{1} The SK starts a TLS session with the model owner and send a device attestation report.
The model vendor verifies device authenticity, encrypts the model topology and parameters with a TLS session key and sends it to SK.
\circled{2} The SK creates a tenant entry in the key storage and stores the encryption and integrity keys.
Each tenant has its own keys similar to the Intel MKTME~\cite{mktme} model and are individually indexed with a unique session ID. 
\circled{3} The tenant configuration registers are populated with base and bound address of the reserved memory locations, scratchpad entries, queue partitions, memory bandwidth allocation and the compute units.
These values are defined through deployment declaration. 
The integrity unit is configured with the integrity granularity obtained from application profiling.
\circled{4} The SK loads the model binary in the instruction memory, the model weights and integrity metadata in respective memory regions.
\circled{5} Next, the SK starts another TLS session with the data owner, sending it the device attestation report with the model hash and the tenant configuration register values.
The data owner verifies the measurement then sends the input over the TLS channel, which is copied by the SK to the input memory region along with any integrity metadata. 

% \vspace{-0.5em}
\subsection{ML inference runtime flow}
\label{subsec:exec_flow}
After the SK completes model and input bootstrapping, the model execution is detailed below:
    \circled{6} The instructions are loaded from the memory to a partitioned instruction queue;
    \circled{7} The decoder sends the \texttt{load} and \texttt{store} instructions to the respective queues, the \texttt{gemm} and \texttt{alu} instructions to the issue queue and the \texttt{zeroize} instructions to the zeroize logic.
    \circled{8} Access-control checks are performed on the memory request addresses before sending them through a constant traffic shaper;
    \circled{9} The received data is decrypted and integrity checked before loading into the corresponding scratchpad.
    \circled{10} Compute instruction resident in the issue queue is executed.
    \circled{11} Dependency queues manage data dependencies between the scratchpads, the compute units, and the zeroize logic to provide functional correctness.
    \circled{12} Dead variables are zeroized in the scratchpad by the zeroize logic.


% \vspace{-1em}


 
\subsection{Encryption and Integrity Engines}
\label{subsec:mem_proc_eng}
Secret data exists as ciphertext outside of the accelerator.
A ciphertext load is decrypted and integrity checked in a staging buffer, inside the memory controller, before transferring it to the scratchpad. 
The staging buffer is partitioned among tenants to avoid data contention.
Tenant-specific keys are retrieved from the key storage for decryption and message authentication code (MAC) verification.
The integrity engine houses partitioned MAC and counter cache to speed up the integrity verification process.
Explicit \texttt{load} and \texttt{store} instructions transact integrity counters and MAC from memory to these caches.
The compiler does not load replay counters for read-only model weights (specified by the API argument discussed in ~\cref{subsec:apis}. 
A single-bit flag in the \texttt{load} instruction is set for read-only data.
The integrity unit performs MAC verification at a granularity decided by profiling and set during application bootstrapping.
It performs MAC verification only after the entire data is loaded into the staging buffer. 
The data is checked for base and bound address before scratchpad transfer.
A dependency queue notifies the compute unit, that the data is ready in scratchpad.


\begin{comment}
The software performs two integrity optimizations:
\textbf{(1)} The read-only model weights do not have replay counters as these values do not change during ML inference.
This optimization reduces the memory bandwidth consumed by metadata loads and also the conflicts in counter cache. 
\textbf{(2)} The software profiles the execution to configure the MAC granularity from $64B$ to $4kB$.
Streaming loads of model layers reduce the memory bandwidth and MAC computation demand with a larger granularity. 
The impact of these two optimizations is reported in~\ref{subsec:eval_integrity}.
The integrity engine houses a configuration register for MAC granularity, that is programmed by SK during tenant bootstrapping.
\end{comment}

\begin{comment}
The memory protection engine (MPE) is in charge of memory encryption, integrity checking,
and access control. 
\cref{fig:mpe} depicts the components of the MPE and how the same hardware can be used for different threat models.
The encryption and integrity engines are configured
with tenant-specific keys by the SK during the model bootstrap time. 
The access control block is configured with the tenant-specific memory and scratchpad bounds.
Every memory requests are checked by the access control block before being sent to the memory. 
The access control block checks for tenant permission to the load/store address as well as the scratchpad location to provide memory isolation among tenants.

The data received via the data bus goes through the multiplexer controlled by the \texttt{privacy bits} which are sent in each \sys{} load/store instruction.
% The secure kernel loads the main memory bounds along with tenant-specific encryption and integrity keys to the tenant selector block during inference bootstrapping.
These bits are $00$ for \textit{public} data and is directly loaded into the scratchpad. 
The lower \texttt{privacy bit} engages the \textit{encryption engine} while the
higher bit engages the \textit{integrity engine}. 
Additional instructions load integrity metadata (MAC and counters) for integrity and freshness guarantees.
There is a metadata cache to hold MAC and counters. 
The integrity engine supports variable granularity ranging from from $64B$ to $4kB$.
The optimal MAC granularity is decided by profiling the ML workload by the \sys{} compiler as detailed in ~\cref{subsec:comp_int_opt}.
The data is temporarily held in the \textit{staging buffers} for integrity verification after which it is loaded to the scratchpad.
The MPE has multiple encryption and integrity engines with each tenant having a dedicated unit including metadata cache and staging buffers.
While all engines work in parallel for a single tenant during temporal sharing to increase the MPE throughput. 
Data stores, also use the same unit to encrypt data, generate integrity metadata and store back to the metadata region in memory.
\end{comment}

% \vspace{-0.5em}
\subsection{Zeroize Module}
\label{subsec:zeroize}

The zeroize logic takes in \texttt{zeroize} instructions, generated from data liveness analysis to overwrite dead secret input, weight and output scratchpad regions.
In addition, it also flushes
the dependency queues and internal buffers during context switch.
The scratchpad write ports are multiplexed between the memory controller and the zeroize module.
The main datapath is prioritized in this multiplexer to prevent pipeline stalls.
The \texttt{zeroize} instructions are decoded and queued in a buffer. 
\sys{} adds dependency queues between the zeroize module
and the compute unit to signal data consumption.
Scratchpad data is zeroized at scratchpad address granularity, which is $256B$ in our implementation.
The output scratchpad is cleared after the data is transferred to the encryption staging buffer.


%\sys{} compiler performs liveness analysis to find out the point of zeroization for each variable. 
%It inserts \texttt{zeroize} instructions at this point of execution. 

%Zeroizing the dead variables proactively frees out scratchpad regions, which can be filled by prefetching future tiles or layers. 
%This also reduces the context switch latency as zeroization is interleaved with the execution. This is possible as the scratchpad as independant read and write ports. 
%The performance benefit of proactive zeroization is discussed in ~\cref{subsec:eval_zeroize}.


\begin{figure}[bt]
    \centering
    \includegraphics[width=0.9\linewidth]{Figures/Traffic shaper.pdf}
    \caption{\textbf{A constant traffic shaper converts memory requests of different data sizes into fixed sized bursts. 
    These bursts are sent at a regular interval, based on the bandwidth declaration. Demand requests are throttled during high demand while fake transactions are inserted in a vacant request queue.}}
    \label{fig:traffic_shaper}
\end{figure}

% \vspace{-0.5em}
\subsection{Constant Traffic Shaper}
\label{subsec:shaper}
A memory traffic shaper converts memory demand requests of variable size into equal-sized transactions.
Each demand request is either split into multiple bursts or padded to create fixed-sized chain of transactions.
These transactions are sent to memory at a fixed interval, which determines the memory bandwidth allocated to the tenant.
\cref{fig:traffic_shaper} shows the demand request conversion inside a traffic shaper. 
The demand requests are stored in tenant-partitioned queues to protect against contention-based side channels.
The transaction splitter performs two operations: 
Firstly, padding smaller transactions ($a$) to a fixed-sized burst ($a'$) 
and splitting larger transactions ($b$) into multiple requests \textbf{($b_1$ , $b_2$)}.
A fake transaction generator fills in fake requests to maintain constant bandwidth during times of no demand. 
Moreover, if the demand request queue fills up, it sends a throttle back to stall request generation. 
An attacker monitoring the memory bus intercepts a constant bandwidth irrespective of the demand request pattern of a victim workload.
A closed row policy in DRAM hides timing difference between row hits and misses, as in Dagguise~\cite{dagguise}. 

\begin{comment}
    

The software profiler chooses the best tile-size based on the user specified bandwidth.
The first profiling pass searches the tile-size state-space to reduce execution time with AutoTVM~\cite{AutoTVM}.
This pass runs the application with different matrix tile combinations. 
Next, the profiler optimizes the generated code by promoting data and metadata load transactions to replace fake transactions with useful data traffic.
The performance and traffic impact of these optimizations are discussed in ~\cref{subsec:eval_shaper}.


\vspace{-1em}






\sarbartha{Overall flow}

\sarbartha{Secure Kernel}

\sarbartha{Memory protection Unit --- Multi-granular integrity}

\sarbartha{Optimized Memory traffic shaper -- Prefetch block against fake transaction}

\sarbartha{Zeroize block -- Proactive zeroization}

\sarbartha{Scratchpad partition -- Access control}

\sarbartha{Queue partition -- Static partition}
\end{comment}


==> evaluation.tex <==
% \vspace{-0.5em}
\section{Implementation}
\label{sec:Implementation}
%-------------------------------------------------------------------------------
First, we enlist the secure accelerator configurations used in our evaluation in ~\cref{subsec:acc_config}.
Next, we introduce the different components of the analytical model in ~\cref{subsec:impl_anal}, 
and the cycle-accurate simulator in ~\cref{subsec:impl_sim}.
Finally, we list the benchmarks used in our evaluation in ~\cref{subsec:impl_bench}.

\subsection{Accelerator configuration}
\label{subsec:acc_config}
The ML inference accelerator is a decoupled-access-execute (DAE) unit with a systolic array implementation. 
Such accelerators are widely used in cloud~\cite{tpuv4} and in edge devices~\cite{vta,eyeriss}.
These accelerators have a fixed dataflow to simplify the hardware design. 
We evaluate with an output-stationary dataflow, used in Google TPUs, but \sys{} can also be used for other dataflows.
The secure blocks comprise of an authenticated encryption unit as shown in ~\cref{fig:hw_arch}, and we use an aes-gcm implementation from prior work~\cite{aes_gcm_num}.
The integrity counters are generated inside the accelerator, as implemented by mgx~\cite{mgx2022isca}.
The secure design also includes a constant traffic shaper, whose bandwidth is programmed during tenant bootstrapping as proposed by sesame~\cite{sesame}. 
It also includes a hardware zeroization unit, taken from sesame, to protect against use-after-free errors. 

We evaluate \sys{} on two secure accelerator designs, with configurations listed in ~\cref{tbl:exp_param}.
The first configuration simulates a cloud MLaaS deployment, while the second smaller configuration simulates an edge deployment of a secure ML accelerator.
The cloud MLaaS design optimization target ($opt_{target}$)is set to minimize the runtime latency, while the edge implementation minimizes performance/watt metric.

%\begin{wraptable}{r}{0.6\linewidth}
 \begin{table}[tp]
    \centering
    \resizebox{0.8\linewidth}{!}{%
   % \ra{1.2}
    \begin{tabular}{|l|cc|}
        \hline
        \textbf{Parameter} &
        \textbf{Cloud MLaaS} & 
        \textbf{Edge Device} \\
        \hline
        %Tenants & 1 & 4 \\
        %\hline
        Memory type & \multicolumn{2}{|c|}{DDR4 @ 3200MHz } \\
        %\hline
        Memory Bandwidth & 128 GB/s & 32 GB/s \\
        %\hline
        Compute units & $256\times256$ &  $64\times64$  \\
        %\hline
        Input Scratchpad & $6144$ KB & $1536$ KB \\
        %\hline
        Weight Scratchpad & $6144$ KB & $1536$ KB \\
        %\hline
        Output Scratchpad & $2048$ KB & $512$ KB \\
        \hline
        %Counter Cache & 128 entries & 32 entries \\
        %\hline
        %MAC Cache & 64 entries & 16 entries \\
        %\hline 
        %Cache properties & \multicolumn{2}{|c|}{Fully-associative Random Repl.} \\
        %\hline
    \end{tabular}
    }
    \caption{\textbf{\sys{} simulator parameters allocated for each tenant in temporal and spatial sharing execution.}}
    \label{tbl:exp_param}
    % \input{Tables/tee_comparison.tex}
\end{table}
%\end{wraptable}


\subsection{Analytical model implementation}
\label{subsec:impl_anal}
The layer tiling and loop order exploration is performed by the gamma~\cite{gamma} mapping tool and the latency and power is estimated with the maestro~\cite{maestro} cost model.
The dataflow is set to output stationary and the offchip bandwidth is set to the crypto block throughput.
We implement a memory trace generator, that takes mapping loop-order and tiles to generate a demand traffic sequence. 
The trace generator inserts the redundant transactions ($T_V$) and integrity hash memory requests ($T_I$), while finding the optimal hash granularity.
The final memory trace is used to estimate the energy consumed during data transfers. 
The traffic shaper sends fixed sized read and write data requests at regular intervals.
The DRAM follows a closed-row policy to service the requests, to prevent response timing from row hits to leak access pattern. 
DRAM power for read and write transactions are taken from DRAMSim3 to compute the energy delay product for different traffic shaper bandwidths. 
The peak occupancy of individual ifmap, weight and ofmap scratchpads for different mappings provide the zeroization latency. 

Finally, the search-space pruner takes the profiling budget in simulation along with the $opt_{target}$ to find the top-m mappings based on ~\cref{alg:two}.
The two parameters that decide the pruning algorithm is the merge factor ($\delta$) and the prune factor ($\epsilon$). 
The merge step clusters layer mappings with similar $opt_{target}$. We use k-means clustering algorithm to combine layer mappings. 
The number of clusters is decided by $\delta$. 
The distance between the different clusters stay the same for different layers. 
Once, mappings are clustered, the mapping having the best $opt_{target}$ is chosen in each clusters. 
A model with $l$ layers and with top-k mappings has a search space of $k^l$.
Assuming that the merging step produces $m_i$ mappings for layer i, the search space is reduced to $\prod_{i=1}^l m_i$.

The next step starts with finding the top cluster for each layer.
The clusters which has a large distance from the top cluster is pruned in this step, based on a prune factor.
The prunefactor becomes more and more aggressive with each iteration, finally giving the top-m model schedules.

%\vspace{-0.5em}
\subsection{Simulator implementation}
\label{subsec:impl_sim}
\sys{} uses the cycle-accurate scale-sim~\cite{scalesim} simulator to evaluate the compiler optimizations.
The simulator is augmented to include the secure hardware.
The authentication unit is simulated with a constant latency added to each memory transaction at the appropriate granularity.
Next, we added a load and a store queue in the traffic shaper to serve as the demand queue as shown in ~\cref{fig:hw_arch}.
These queues are of finite size as listed in ~\cref{tbl:exp_param} and stalls the system during times of high demand. 
The traffic shaper also sends a fake transaction every time the demand queue is empty. 
Finally, we add a zeroize block, that shares the scratchpad write port with the main data pipeline. 
It contains a queue holding zeroize instructions, similar to the sesame implementation and zeroizes a 
scratchpad line (256 Bytes), when the read port is free. 
The DRAM transactions are simulated with the ramulator~\cite{ramulator} tool.
The arrival time of each transaction is added to the request dispatch simulator tick.

The simulator is fed with a model binary, generated by the compiler. The \texttt{load} and \texttt{store} instructions are loaded into the respective traffic shaper demand queue. The \texttt{gemm} instructions are simulated by the compute unit, and the \texttt{zeroize} instruction zeroizes specific regions of a scratchpad. The simulator also keeps track of data dependencies to ensure correctness.


\begin{comment}
    

The scale-sim simulator is augmented to include an instruction queue and a decoder.
The model binary is loaded into the instruction queue. 
The load/store queue, the compute issue queue and the zeroize queue, described in ~\cref{subsec:exec_flow} is added to the simulator. 
The decoder adds stall cycles, if any of the queues are full and waits for the existing instructions to complete.
The accelerator memory controller is designed to include separate constant traffic shapers for read and write buses and 
timing models for encryption and integrity units. 
Encryption and integrity verification computation times are taken from prior work~\cite{aes_gcm_num}.
The transactions generated by the traffic shaper is fed to ramulator.
The ramulator emits arrival time for each transaction, which is added as memory latency to the simulator clock.
The zeroize logic polls the compute dependency queue and the scratchpad write port to zeroize secret data. 
The system is back-pressured by finite queue sizes listed in~\cref{tbl:exp_param}.
\end{comment}
%The constant traffic shaper sends the memory requests at regular intervals to the ramulator. 
%The ramulator reports the arrival time of each transaction after which it is loaded to the staging buffer for decryption and integrity verification.
%The encryption unit is a timing model. Encryption and decryption cycles are added before the data is ready for scalesim.
%This cycles are taken from a prior implementation~\cite{aes_gcm_num}. 
%The integrity engine verifies the MAC with metadata (counters and MAC), either present in the respective metadata cache or loaded from memory.
%The data is then made available to the scratchpad and the dependency queue is cleared for computation.

%Once, the output is generated, it is encrypted and a new MAC is generated. The data along with the MAC is stored back to memory by the traffic shaper. The zeroize logic clears the scratchpad region holding stale data. 


\begin{comment}
The memory controller is designed to include encryption and integrity block along with a constant traffic shaper as explained in \cref{sec:overview}. 
The integrity unit has caches individually for storing counters and MAC. 
Memory is simulated using the ramulator~\cite{ramulator} tool.
Memory transactions are sent to the ramulator based on the demand request generated by scale-sim and a timing model computes the data arrival latency. Memory requests are also back-pressured in the request queue inside the memory controller. 

\begin{figure}[t]
%\begin{wrapfigure}{r}{0.8\linewidth}
    \centering
    \includegraphics[width=\linewidth]{Figures/Scalesim_config.drawio.pdf}
    \caption{\textbf{\sys{} cycle-accurate simulator}}
    \label{fig:simulator}
%\end{wrapfigure}
\end{figure}

The scale-sim simulator is modified to accept compute instructions instead of pre-defined model topology files. 
The compute instructions are issued only when data is ready in the input and weight scratchpads.
Each of the scratchpads have one read and one write port. The write port is multiplexed between memory controller
and the zeroize module.

The DMA engine sends shaped requests to the Ramulator which returns the cycle at which the transaction is completed. 
Encryption and integrity computation are simulated as a timing model with delays taken from an hardware implementation on Xilinx FPGA~\cite{aes_gcm_num}.
The integrity MAC and counter loads are first looked up in metadata cache.
A load request is sent to the memory controller in case of a metadata miss.
\end{comment}
\vspace{-0.5em}


\subsection{Benchmarks}
\label{subsec:impl_bench}
Benchmarks are chosen to evaluate different types of ML models.
This includes applications like image classification -- \textbf{Alexnet}~\cite{alexnet} and \textbf{Resnet-50}~\cite{resnetv2};
object detection -- \textbf{FasterRCNN}~\cite{fasterrcnn},
recommendation systems -- \textbf{DLRM}~\cite{DLRM},
a gaming bot -- \textbf{AlphaGoZero}~\cite{AlphaGoZero},
the encoding layer of a LSTM language translation model -- \textbf{Translate}~\cite{translate},
a basic transformer with text embeddings -- \textbf{Transformer}~\cite{Transformer}.


\section{Evaluation}
In this section, we evaluate \sys{} and quantify the secure ML inference overhead compared to a non-secure baseline.
First, we break down the execution overhead for each defense mechanism for both \textit{temporal} and \textit{spatial} scenarios, described in ~\cref{subsec:overhead_analysis}. 
Next, we show the benefits of each compiler optimization in \cref{subsec:perf_opt_eval}.
Finally, we report the security evaluation of the optimized implementation in ~\cref{subsec:net_overhead}.
We exclude the bootstrapping time in our evaluation and only focus on the ML inference execution latency.
\vspace{-0.5em}
\subsection{Latency Overhead Breakdown}
\label{subsec:overhead_analysis}

The grey bar shows the ML inference latency overhead in~\cref{fig:overhead_most_secure} and the adjacent bar shows the overhead contribution of each defence mechanism. 
The compiler optimization and profiling is not performed in this secure inference. 
However, this execution guarantees the security properties of \sys{} and we use it as our \textit{baseline} secure system.
The overhead is normalized to the non-secure execution latency for temporal and spatial modes respectively.
%---proactive zeroization, fake transaction reduction, and
%integrity size customization.
The average execution overhead is $1.95\times$ in the temporal sharing and $2.07\times$ in the spatial sharing mode. 
The encryption overhead is due to the data pipeline stalls for each data encryption and decryption.
The overhead is proportional to the model size, with larger models like \textit{Translate} and \textit{Transformer} having the maximum overhead.
% A stream cipher, instead of a block cipher algorithm, could improve the encryption overhead, but we leave this analysis to future work.

The integrity overhead includes the extra memory transactions for fetching MAC and counters and 
extra computation latency for integrity verification.
The $64B$ MAC granularity introduces additional memory transactions over an already constrained memory bus.
Spatial sharing encounters ever larger overhead due to $>95\%$ average occupancy of metadata caches.
\textit{DLRM} overhead exceeds more than $2\times$ in spatial mode due to large metadata traffic and stall in the metadata caches.

The memory traffic shaper increases latency by throttling the demand transactions for larger layers. 
ML workloads with small layers (\textit{Resnet50, FasterRCNN, Translate, and Transformer}) generate considerable fake transactions.
The real transactions are delayed due to in-flight fake transactions.
Optimizing the traffic shaper is essential to reduce energy and memory traffic overhead caused by fake transactions.

%Performing data integrity checks on such large data volumes delay execution.
In this experiment, we do not use the zeroize module, but flush the scratchpad during a context switch.
The temporal models have a larger zeroization overhead due to larger scratchpad occupancy by a tenant. 

%Moreover, traffic shaper also adds significant network traffic stalling the memory bus in certain cases.
%Finally, there is an overhead associated with data encryption and decryption. 
% Since, the contribution of this overhead is much smaller, we do not perform any optimizations on data encryption in this paper.
%However, changing the encryption scheme or deploying stream encryption can reduce this overhead which will be addressed in a future work.
Another interesting thing to note in ~\cref{fig:overhead_most_secure} is that,
the overall execution overhead (first bar) with all the security widgets is greater than the sum of its parts (second bar).
This is due to additional stalls introduced by the runtime inter-dependency among these secure hardware components.
The only exception is \textit{Translate} in spatial sharing.
This is due to the overlap in stall cycles among the defense mechanisms.
%Reducing individual overheads with domain-specific optimizations will reduce stalls between security widgets
%as we illustrate in the next sections.
\vspace{-0.5em}
\subsection{Performance Optimizations}
\label{subsec:perf_opt_eval}
In this section, we evaluate the performance optimizations enabled by the \sys{} compiler.
% The majority of overhead for secure execution comes from memory integrity and scratchpad zeroization. 
Specifically, we will see how
integrity optimizations (\cref{subsec:eval_integrity}),
proactive zeroization (\cref{subsec:eval_zeroize}),
and
fake transaction reduction (\cref{subsec:eval_shaper})
reduce secure execution overhead. 
% \sarbartha{Remove remaining text... Just left for comments}
% % to reduce the performance overhead introduced by memory integrity, constant traffic shaper and secret zeroization. 
% In this section, we evaluate some of\todo{we should evaluate all optimizations used right? which one did we leave out?}
% \sarbartha{Rephrased}
% the optimizations in the context of a temporally shared accelerator. 
% Same study is also performed for spatial sharing but is not included due to space constraints.\todo{can we add a comment stating results/trends are similar? Or summarize the take-aways from that analysis...Any surprises?}
% \sarbartha{I will add plots for spatial sharing for integrity and add a row in the table for zeroization}

\subsubsection{Integrity optimizations}
\label{subsec:eval_integrity}
\begin{figure}[t]
    \centering
    \hspace{-1em}
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\linewidth]{Figures/integrity_temporal.png}
        \vspace{-1em}
        \caption{Temporal multi-tenancy}
        \label{fig:temporal_integrity}
    \end{subfigure}
    \begin{subfigure}{0.5\linewidth}
        \includegraphics[width=\linewidth]{Figures/integrity_spatial.png}
        \vspace{-1em}
        \caption{Spatial multi-tenancy}
        \label{fig:spatial_integrity}
    \end{subfigure}
    \caption{\textbf{Performance overhead reduced by optimizing integrity granularity (normalized to a non-secure baseline).}}
    \vspace{-1em}
    \label{fig:integrity_opt}
\end{figure}
%\begin{figure}[t]
%    \centering
%    \includegraphics[width=0.5\linewidth]{Triton_asplos/Figures/integrity_temporal.png}
%    \caption{\textbf{Performance overhead reduced by optimizing integrity granularity (normalized to a non-secure baseline).}}
%    \label{fig:integrity_opt}
%\end{figure}
 
\sys{} compiler performs two integrity optimizations (\cref{subsec:mem_proc_eng}):
\textbf{(1)} Freshness counters are omitted for read-only model weights and 
\textbf{(2)} The integrity verification granularity is tailored to each application.
% \todo{the compiler sets the granularity right? So it is not runtime? but just tailored to applications}
%Moreover, customizing the granularity of integrity protection to the tile datasize reduces the number of integrity checks.
%This is helpful in ML workloads where a large chunk of consecutive
%memory locations is loaded together before computation commencement. 
%Since, the model and input size is known beforehand, the compiler
%can optimize the integrity granularity for each workload.
The first bar in \cref{fig:integrity_opt} shows the execution overhead with a $64B$ integrity granularity. 
The second bar (\textit{$opt\_64$}), shows the performance improvement due to integrity counter exclusion of read-only model weights.
There is an average performance overhead reduction of $18.2\%$ in temporal sharing and $10.1\%$ overhead reduction in spatial sharing with this domain-specific optimization.
Models like \textit{FasterRCNN} and \textit{AlphaGoZero} show more than $25\%$ latency reduction in temporal sharing due to less conflict misses in the counter cache.
Spatial sharing models benefit less due to already constrained memory bandwidth and smaller MAC cache size per tenant.

Next, the compiler profiling of different MAC granularities ($64B$ to $4kB$) is shown in the remaining bars.
The optimum granularity is mentioned for each application in the plot.
Models with larger tile sizes, like \textit{DLRM} and \textit{Transformer} benefit from larger MAC granularity in temporal sharing mode but starts giving diminishing returns beyond $1024B$.
Large granularity are also sub-optimal for workloads with inputs that are either small or have a strided pattern (\textit{Resnet50} and \textit{FasterRCNN}).
All the workloads prefer higher granularity in the spatial mode due to limited MAC and counter cache sizes.
Overall, integrity optimizations reduce the performance overhead ranging from $8\%$ for \textit{Alexnet} to $93\%$ for \textit{FasterRCNN} in temporal sharing mode. 
The corresponding spatial overhead reduction ranges from $4\%$ for \textit{Translate} to $261\%$ for \textit{DLRM}.  


\subsubsection{Proactive zeroization}
\label{subsec:eval_zeroize}

The \textit{regular} bar in ~\cref{fig:proactive_zero} illustrates the latency overhead from secret zeroization. 
The secrets are zeroized at the end of each layer in temporal sharing.
For spatial sharing, the secrets are zeroized at the end of execution. 
The \textit{proactive} bar performs data liveness analysis and proactively zeroizes dead variables with explicit \texttt{zeroize} instructions. 
The zeroize hardware interleaves these instructions with the inference computation.
This reduces the left-over secrets at the end of execution.
This latency overhead is reduced from $23.15\%$ to $10.36\%$ for temporal sharing and from $10.61\%$ to $6.90\%$ for spatial sharing with the proactive zeroization technique.
Compute-intensive models like $DLRM$ and $AlphaGoZero$ benefit from proactive zeroization. 
The memory load pipeline is stalled during compute cycles due to large scratchpad occupancy.
The scratchpad write port is efficiently utilized by the zeroize module during computation.
The temporal overhead reduction is more than spatial due to the larger scratchpad allocation to a tenant. 
The number of scratchpad locations, that need to be zeroized during context switch is higher in temporal sharing mode.

\begin{comment}
Proactively identifying dead variables and zeroizing them during execution reduces the average geometric overhead ranging
from .
Interleaving zeroization with computation of later layers amortizes context switch latency.
Proactive zeroization increases the density of useful data in the scratchpad.
It replaces the fake transactions for smaller layers with useful data and metadata prefetches, reducing effective data load latency. 
\end{comment}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/proactive_zeroize.pdf}
    \caption{ \textbf{The \textit{Regular} bar shows the latency overhead with zeroization during a context switch.
    The \textit{Proactive} bar shows the latency reduction with \texttt{zeroize} instructions generated from liveness analysis and issued by the zeroize module.}}
    \label{fig:proactive_zero}
\end{figure}
% \todo{are we able to show how much percentage of the zeroization operations can be made proactive?}
% \sarbartha{Need to go back and check the results. TBD}
\begin{comment}
    

 \begin{table*}[h]
    \resizebox{\linewidth}{!}{
    \begin{tabular}{|l|c|c|c|c|c|c|c|c|}
        \hline
        \textbf{Zeroization} & \textbf{Alexnet} & \textbf{Resnet50} & \textbf{FasterRCNN} & \textbf{DLRM} & \textbf{AlphaGoZero} & \textbf{Translate} & \textbf{Transformer} & \textbf{Geo\_mean} \\
        \hline
         \textbf{Regular} & 9.22 & 34.69 & 32.19 & 39.47 & 23.05 & 19.67 & 19.33 & 23.15 \\
        \hline
        \textbf{Proactive} & 7.85 & 15.31 & 14.62 & 23.61 & 6.27 & 10.83 & 7.46 & 10.36 \\
        \hline
    \end{tabular}
    }
    \caption{Performance overhead (in $\%$) comparison between regular and proactive zeroization in the temporal sharing mode}
    \label{tbl:proactive_zeroization}
    % \input{Tables/tee_comparison.tex}
   \vspace{-1em}
\end{table*}
\end{comment}

\subsubsection{Fake traffic reduction}
\label{subsec:eval_shaper}

\begin{comment}
\begin{figure*}[htbp]
    \centering
    \includegraphics[width=\linewidth]{Figures/memory_traffic_analysis.png}
    \caption{Fake memory traffic and corresponding inference latency comparison for different memory bandwidth allocations. }
    %Orange portion  --- Resultant optimized fake memory traffic and inference latency. Pink portion -- Improvement from data prefetch; Grey portion --- Improvement from metadata prefetch.}
    \label{fig:shaper_study}
    \vspace{-1em}
\end{figure*}
\end{comment}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/shaper_traffic.pdf}
    \caption{ \textbf{Percentage of fake traffic converted to useful metadata or real data transactions. 
    The black bar shows the latency reduction normalized to the non-secure baseline.}
    }
    \label{fig:shaper_study}
\end{figure}

\sys{} compiler reduces the number of fake transaction in the traffic shaper by prefetching real and metadata requests.
This is done by promoting \texttt{load} instructions of subsequent layers in the binary by the compiler.
The positive y-axis in the \cref{fig:shaper_study} demonstrates the number of fake transactions that are converted to real data (purple) and metadata (pink) transactions.
Models with larger layers like \textit{Alexnet, DLRM} and \textit{AlphaGoZero} have limited scratchpad availability. 
They benefit much more from metadata prefetch in temporal sharing mode. 
The small layers in \textit{Translate} and \textit{Transformer} benefit from loading subsequent layers in the scratchpad. 
The number of metadata transactions is higher in temporal sharing mode due to larger metadata cache availability. 
On average, $20.56\%$ of fake transactions are converted into useful transactions in temporal sharing mode, providing a latency improvement of $7.68\%$.
In spatial sharing mode, $12.84\%$ of fake transactions are reduced, while providing a latency improvement of $2.7\%$ compared to non-secure baseline. 
Even though the benefit of this optimization is less in spatial sharing mode, it reduces memory traffic in a more constrained memory bus.
Reducing the number of fake transactions also improves the overall energy consumed by the secure ML inference accelerator.
\vspace{-0.5em}
\subsection{\sys{} net latency improvement}
\label{subsec:net_overhead}
Each of the defense optimizations yields secure ML inference latency reduction. 
~\cref{fig:latency} shows the overall latency of secure inference for \sys{} compared to the baseline (demonstrated in ~\cref{fig:overhead_most_secure}), normalized to a non-secure baseline.
The availability of more resources in the temporal sharing mode provides greater optimization scope. 
The baseline secure platform has a performance overhead of $2.04\times$ the non-secure inference.
\sys{} reduces the overhead to $1.41\times$ with the same security policy. 
\sys{} not only improves integrity verification, traffic shaper and the zeroize logic performance, but also reduces inter-dependency stalls.
Having more useful data in the scratchpad reduces the number of compute stalls in ML inference. 
Since, the evaluation assumes a  context switch after each layer, deeper models like \textit{Translate} and \textit{Transformer} still have a large overhead. 
In reality, multi-tenant ML accelerators perform much fewer context switches, 
which will reduce the execution overhead even further.
%this is an over-approximation in multi-tenant environment and the number of context switches will be much less, leading to a lower overhead. 
Moreover, a stream cipher will reduce the encryption overhead and is left for future work.

The spatial overhead is reduced from $2.13\times$ to $1.46\times$.
The largest overhead reduction is observed in $DLRM$, which benefits from a larger integrity granularity and less cache conjestion due to read-only data declaration, reducing the overhead from $4.55\times$ to $1.53\times$. 
In general, DLRM has large layers and is not a good fit for the spatially partitioned accelerator. 
The user can use the \sys{} profiling to define the deployment declaration and resource allocation for an application. 
This helps the developer to make an informed resource declaration for each application.
%\sarbartha{Elaborate on other benchmarks}


\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{Figures/obsidian_latency.pdf}
    \caption{\textbf{Secure ML inference latency comparison between the baseline and \sys{}.}}
    \label{fig:latency}
    \vspace{-0.5em}
\end{figure}



\begin{comment}
    

We perform a sensitivity study to observe the amount of fake transactions generated, when a tenant is allocated different bandwidths in the temporal sharing mode.
We run each benchmark by tuning the allocated memory bandwidth ($BW_c$) to five configurations (128, 100, 72, 48, 24GB/s).
~\cref{fig:traffic_shaper} shows the number of fake transactions and the associated inference latency when the tenant is allocated bandwidths of
$100\%$, $80\%$, $60\%$, $40\%$ and $20\%$ of the total memory bandwidth.
The obvious observation is that, the number of fake transactions decrease with 


The total number of fake transaction is a function of inference latency and the allocated bandwidth.
The allocated bandwidth is the dominant factor to decide the number of fake transactions.
However, the higher inference latency at $80\%$ bandwidth produces more fake transactions than 
However, $DLRM$, $AlphaGoZero$ and $Translate$ has more fake transactions at $80\%$ bandwidth due to the inference latency dominating 



The number of fake transactions and the inference latency associated with it is shown in~\cref{fig:temporal_overhead_analysis}.
The first bar illustrates the case, where the entire memory bandwidth is allocated 

The overhead incurred by the traffic shaper described in~\cref{fig:temporal_overhead_analysis} is with the entire allocated memory bandwidth and is the baseline for this sensitivity study.
Intuitively, shaping traffic to the max allocated memory bandwidth leads to
a large amount of fake transactions when there is low or no demand.
The overhead arises when $BW_d > BW_c$  leading to either memory request throttles
or demand requests waiting behind in-flight fake transactions.
\cref{fig:shaper_study} illustrates the trade-off between the amount of fake memory traffic and the system performance. 

The fake memory traffic reduces with memory allocation in most cases.
However, the reduction in memory bandwidth can introduce execution stall increasing the overall execution time and the number of fake transactions.
The developer can either choose a specific bandwidth or the \sys{} framework can choose the optimum bandwidth based on \texttt{exec\_time} input.

Each bar in the left plot of \cref{fig:shaper_study} is the fake transaction volume without any shaper optimizations. 
Bars in the right plot report the latency normalized to the non-secure ML inference.
The grey portion in each bar is the fake traffic that can be replaced with useful metadata prefetching (counters and MAC). This leads to a corresponding latency reduction shown in the right plot.
The pink portion of the graphs represent the additional fake traffic reduction by data prefetching
from subsequent tiles or even layers into free scratchpad region created by proactive zeroization.
The fake traffic volume and the inference latency after the two optimizations is shown in the orange portion.
These optimizations reduce the fake traffic ranging from $7.29\%$ to $27.59\%$ and a latency ranging from $2.25\%$ to $18.34\%$.


\sarbartha{Basic overhead of secure ML accelerator}

\sarbartha{improvement from integrity granularity}

\sarbartha{Improvement from traffic shaper}

\sarbartha{Improvement from proactive zeroizer}

\sarbartha{Overall overhead}

\sarbartha{Area numbers}
\end{comment}


==> threat_model.tex <==
\newtcolorbox{cbox}[1]{%
width=\columnwidth,%
before skip=0.3em, after skip=0.1em,%
left=0.4mm,right=0.4mm,top=0.4mm,bottom=0.4mm,arc=1mm,%
boxsep=1mm,boxrule=1pt,fonttitle=\bfseries,title={#1},%
colback=white,colframe=gray!30!,coltitle=black
}

\section{Threat model and goals}
%First, we define the secret data assets during ML inference. 
%Subsequently, the platform assumptions are enlisted.
%Finally, we define the threat model for both spatial and temporal secure execution.

\subsection{Data assets}
ML inference takes in an ML model and a data input to produce a classification output. 
The goal of \sys{} is to protect the value of the model weights, the data input and the output.
The ML model is a sequence of layers, where the intermediate output is the input to a subsequent layer.
These outputs (feature vectors) are large to fit in the accelerator for some layers and is stored back to memory.
\sys{} needs to protect these intermediate features as they contain signatures of the data input and the corresponding ML layer. 

The other asset that \sys{} protects, is the ML model topology and the size of the inputs, outputs and the feature vectors. 
Prior work~\cite{ReverseCNN, band_util} reverse-engineered an ML model from its layer structure, using black-box attacks.
%The attacker can also decipher the secret inputof the input and output size.
The matrix or vector structure is visible to an attacker through the knowledge of main memory allocation, 
the memory bandwidth utilization and the on-chip scratchpad or buffer contention.


\begin{comment}
ML inference executes user input data with a confidential model IP to produce a classification.
Input/output data values and model weights are the data assets that need confidentiality and integrity protection. 
Intermediate variables generated during computation, also require similar protection.
Moreover, the input data structure and the model topology are also confidential information. 
Prior work~\cite{ReverseCNN, band_util} reverse-engineered an ML model from topology information. 
Moreover, in certain inference applications like language translation,
prior work extracted the input text from the input size.
\end{comment}
\vspace{-0.5em}
\subsection{Assumptions}
We list certain assumptions, some of which are fundamental, while others, being demonstrated by prior work.
We trust the accelerator manufacturer and assume its components are free from hardware trojans.
A manufacturer-provisioned key, stored in a secure storage, signs the device attestation report.
\sys{} relies on a standard remote attestation flow described in prior works~\cite{shef,GuardNN2022DAC}
for attesting the authenticity of the accelerator hardware and firmware.
A provisioning processor (described in ~\cref{subsec:secure_kernel}), performing the remote attestation and providing
the accelerator interface to a tenant, is safeguarded with secure boot.
The \sys{} compiler code is assumed to be a part of our trusted computing base (TCB).
The formal verification of \sys{} compiler is left for future work.
\vspace{-0.5em}
\subsection{Threat model}
We assume a powerful attacker, who can share temporal slice with victim execution or co-execute with the victim in a spatial multi-tenant environment.
An attacker cannot observe and tamper secret data in main memory, during data transfer and inside the accelerator.
Moreover, an attacker cannot infer secret data size from the demand memory requests and from resource allocation.
The attacker cannot contend with victim's reserved scratchpad, dependency queues, memory requests, instructions and compute units.
Furthermore, an attacker can observe or prime scratchpads or accelerator buffers, before and after victim execution, but cannot decipher any secret data.
%The attacker can observe and tamper with micro-architectural components like scratchpad, various queues--dependency, memory request, instruction, and issue.
%Moreover, the attacker can launch side-channel attacks such as 
%contention side channels on the victim queues, scratchpad utilization, compute units,
%and termination timing side channels.
%The attacker can occupy the entire accelerator before and after the victim's execution 
%to monitor the victim's left-over state and data in memory, queues, and SRAM.

However, we assume that the trained model is not susceptible to algorithmic and data poisoning attacks~\cite{poisoning_1,poisoning_2,poisoning_3}. 
Finally, denial-of-service (DoS), power, and electromagnetic side-channels as out-of-scope for this work.
\vspace{-0.5em}
\subsection{Security Properties}
\label{subsec:sec_prop}
\begin{cbox}{S1. Data Value Confidentiality}
The model weights, the inference inputs, the intermediate feature vectors, and the output should be kept secret from other tenants.
\end{cbox}
\textbf{Requirement:} Training a model requires considerable time, computing resources, and a large data corpus.
Hence, it is important to safeguard the confidentiality of model weights from an attacker.
Inference inputs and intermediate feature vectors contain user private data and hence are confidential in secure ML inference.

\begin{cbox}{S2. Data Integrity}
The integrity of the ML model, inference input, the intermediate feature vectors, and the output should be safeguarded.
\end{cbox}
\textbf{Requirement:} Tampering the ML model weights and the inference input can change the inference outcome.
This enables the attacker to change the classification or generate toxic content. 
Moreover, the ML inference should be resistant from data replay attacks.

\begin{cbox}{S3. Data structure confidentiality}
The model layer structure and the size of the inference input and output
are confidential.
\end{cbox}
\textbf{Requirement:} The size of the input or classification output can violate data confidentiality. 
For instance, the size of an input and output sentence can correlate with its content. 
Similarly, an attacker can break model confidentiality by initiating black box attacks. 
Black box attacks are possible with layer structure knowledge as demonstrated by prior works~\cite{black_box},

==> zeroize_algo.tex <==
\begin{algorithm}
\caption{An algorithm with caption}\label{alg:two}
\KwInput{$L_1, L_2, ..., L_n $}
\KwResult{$y = x^n$}
$y \gets 1$\;
$X \gets x$\;
$N \gets n$\;
\While{$N \neq 0$}{
  \eIf{$N$ is even}{
    $X \gets X \times X$\;
    $N \gets \frac{N}{2}$ \Comment*[r]{This is a comment}
  }{\If{$N$ is odd}{
      $y \gets y \times X$\;
      $N \gets N - 1$\;
    }
  }
}
\end{algorithm}
